ScheduleNet: Learn to solve multi-agent scheduling problems with reinforcement learning

We propose ScheduleNet, a RL-based real-time scheduler, that can solve various types of multi-agent scheduling problems. We formulate these problems as a semi-MDP with episodic reward (makespan) and learn ScheduleNet, a decentralized decision-making policy that can effectively coordinate multiple agents to complete tasks. The decision making procedure of ScheduleNet includes: (1) representing the state of a scheduling problem with the agent-task graph, (2) extracting node embeddings for agent and tasks nodes, the important relational information among agents and tasks, by employing the type-aware graph attention (TGA), and (3) computing the assignment probability with the computed node embeddings. We validate the effectiveness of ScheduleNet as a general learning-based scheduler for solving various types of multi-agent scheduling tasks, including multiple salesman traveling problem (mTSP) and job shop scheduling problem (JSP).

==> packages_old.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\newcommand{\Tau}{\mathrm{T}}
\usepackage{xcolor}         % colors
% \usepackage{graphicx}

% \usepackage{multirow}
\usepackage{makecell}
\usepackage{enumitem}
\usepackage{amsmath}
% \usepackage{color,soul}
\usepackage{enumitem}
% \usepackage{booktabs} % for professional tables
% \usepackage{bbm}
% \usepackage{algorithm} 
% \usepackage{algpseudocode} 
\usepackage{adjustbox}  
% \usepackage{wrapfig,lipsum,booktabs}
\usepackage{amssymb}
\input{math_command.tex}
% \usepackage{wrapfig}

% subfigures
% \usepackage{subfig}
% \usepackage{subcaption}
\usepackage{caption}
% \usepackage{multicol}

% Algorithm chart
\usepackage[ruled,linesnumbered]{algorithm2e}

% \usepackage{stmaryrd}
% \DeclareMathOperator*{\VERT}{\Big\Vert}

% Citation related
\usepackage[square, numbers]{natbib}
\bibliographystyle{abbrvnat}
